An Empirically Evaluated Checklist for Surveys in Software Engineering

Context: Over the past decade Software Engineering research has seen a steady increase in survey-based studies, and there are several guidelines providing support for those willing to carry out surveys. The need for auditing survey research has been raised in the literature. Checklists have been used to assess different types of empirical studies, such as experiments and case studies. Objective: This paper proposes a checklist to support the design and assessment of survey-based research in software engineering grounded in existing guidelines for survey research. We further evaluated the checklist in the research practice context. Method: To construct the checklist, we systematically aggregated knowledge from 14 methodological papers supporting survey-based research in software engineering. We identified the key stages of the survey process and its recommended practices through thematic analysis and vote counting. To improve our initially designed checklist we evaluated it using a mixed evaluation approach involving experienced researchers. Results: The evaluation provided insights regarding limitations of the checklist in relation to its understanding and objectivity. In particular, 19 of the 38 checklist items were improved according to the feedback received from its evaluation. Finally, a discussion on how to use the checklist and what its implications are for research practice is also provided. Conclusion: The proposed checklist is an instrument suitable for auditing survey reports as well as a support tool to guide ongoing research with regard to the survey design process.

==> references <==
@inproceedings{perry2000empirical,
  title={Empirical studies of software engineering: a roadmap},
  author={Perry, Dewayne E and Porter, Adam A and Votta, Lawrence G},
  booktitle={Proceedings of the conference on The future of Software engineering},
  pages={345--355},
  year={2000},
  organization={ACM}
}

@inproceedings{sjoberg2007future,
  title={The future of empirical methods in software engineering research},
  author={Sjoberg, Dag IK and Dyba, Tore and Jorgensen, Magne},
  booktitle={2007 Future of Software Engineering},
  pages={358--378},
  year={2007},
  organization={IEEE Computer Society}
}

@inproceedings{wohlin2016there,
  title={Is there a Future for Empirical Software Engineering?},
  author={Wohlin, Claes},
  booktitle={Proceedings of the 10th ACM/IEEE International Symposium on Empirical Software Engineering and Measurement},
  pages={1},
  year={2016},
  organization={ACM}
}

@article{cohen1968weighted,
  title={Weighted kappa: Nominal scale agreement provision for scaled disagreement or partial credit.},
  author={Cohen, Jacob},
  journal={Psychological bulletin},
  volume={70},
  number={4},
  pages={213},
  year={1968},
  publisher={American Psychological Association}
}

@inproceedings{perry2004case,
  title={Case studies for software engineers},
  author={Perry, Dewayne E and Sim, Susan Elliott and Easterbrook, Steve M},
  booktitle={Software Engineering, 2004. ICSE 2004. Proceedings. 26th International Conference on},
  pages={736--738},
  year={2004},
  organization={IEEE}
}

@techreport{kasunic2005designing,
  title={Designing an effective survey},
  author={Kasunic, Mark},
  year={2005},
  institution={CMU/SEI-2005-HB-004.
Software Engineering Institute, Carnegie Mellon University.}
}

@inproceedings{molleri2018teaching,
  title={Teaching students critical appraisal of scientific literature using checklists},
  author={Moll{\'e}ri, Jefferson Seide and bin Ali, Nauman and Petersen, Kai and Minhas, Nasir Mehmood and Chatzipetrou, Panagiota},
  booktitle={Proceedings of the 3rd European Conference of Software Engineering Education},
  pages={8--17},
  year={2018},
  organization={ACM}
}

@inproceedings{Wieringa12,
  author    = {Roel Wieringa},
  title     = {Towards a unified checklist for empirical research in software engineering:
               first proposal},
  booktitle = {16th International Conference on Evaluation {\&} Assessment in
               Software Engineering, {EASE} 2012, Ciudad Real, Spain, May 14-15,
               2012. Proceedings},
  pages     = {161--165},
  year      = {2012},
}

@article{kitchenham1995case,
  title={Case studies for method and tool evaluation},
  author={Kitchenham, Barbara and Pickard, Lesley and Pfleeger, Shari Lawrence},
  journal={IEEE software},
  volume={12},
  number={4},
  pages={52--62},
  year={1995},
  publisher={IEEE}
}

@article{KitchenhamBTNLPB10,
  author    = {Barbara A. Kitchenham and
               Pearl Brereton and
               Mark Turner and
               Mahmood Niazi and
               Stephen G. Linkman and
               Rialette Pretorius and
               David Budgen},
  title     = {Refining the systematic literature review process - two participant-observer
               case studies},
  journal   = {Empirical Software Engineering},
  volume    = {15},
  number    = {6},
  pages     = {618--653},
  year      = {2010},
}

@inproceedings{DybaD08,
  author    = {Tore Dyb{\aa} and
               Torgeir Dings{\o}yr},
  title     = {Strength of evidence in systematic reviews in software engineering},
  booktitle = {Proceedings of the Second International Symposium on Empirical Software
               Engineering and Measurement, {ESEM} 2008, October 9-10, 2008, Kaiserslautern,
               Germany},
  pages     = {178--187},
  year      = {2008},
}

@article{dybaa2008empirical,
  title={Empirical studies of agile software development: A systematic review},
  author={Dyb{\aa}, Tore and Dings{\o}yr, Torgeir},
  journal={Information and software technology},
  volume={50},
  number={9},
  pages={833--859},
  year={2008},
  publisher={Elsevier}
}

@inproceedings{KitchenhamSBBDHPR10,
  author    = {Barbara Kitchenham and
               Dag I. K. Sj{\o}berg and
               Pearl Brereton and
               David Budgen and
               Tore Dyb{\aa} and
               Martin H{\"{o}}st and
               Dietmar Pfahl and
               Per Runeson},
  title     = {Can we evaluate the quality of software engineering experiments?},
  booktitle = {Proceedings of the International Symposium on Empirical Software Engineering
               and Measurement, {ESEM} 2010, 16-17 September 2010, Bolzano/Bozen,
               Italy},
  year      = {2010},
}

@article{consort2010statement,
  title={CONSORT 2010 statement: updated guidelines for reporting parallel group randomised trials},
  author={Schulz, Kenneth F and Altman, Douglas G and Moher, David},
  journal={BMC medicine},
  volume={8},
  number={1},
  pages={18},
  year={2010},
  publisher={BioMed Central}
}

@inproceedings{JedlitschkaP05,
  author    = {Andreas Jedlitschka and
               Dietmar Pfahl},
  title     = {Reporting guidelines for controlled experiments in software engineering},
  booktitle = {2005 International Symposium on Empirical Software Engineering {(ISESE}
               2005), 17-18 November 2005, Noosa Heads, Australia},
  pages     = {95--104},
  year      = {2005},
}

@inproceedings{WieringaCDMP12,
  author    = {Roel Wieringa and
               Nelly Condori{-}Fern{\'{a}}ndez and
               Maya Daneva and
               Bela Mutschler and
               Oscar Pastor},
  title     = {Lessons learned from evaluating a checklist for reporting experimental
               and observational research},
  booktitle = {2012 {ACM-IEEE} International Symposium on Empirical Software Engineering
               and Measurement, {ESEM} '12, Lund, Sweden - September 19 - 20, 2012},
  pages     = {157--160},
  year      = {2012},
}

@inproceedings{HostR07,
  author    = {Martin H{\"{o}}st and
               Per Runeson},
  title     = {Checklists for Software Engineering Case Study Research},
  booktitle = {Proceedings of the First International Symposium on Empirical Software
               Engineering and Measurement, {ESEM} 2007, September 20-21, 2007, Madrid,
               Spain},
  pages     = {479--481},
  year      = {2007},
}

@article{malhotra1998assessment,
  title={An assessment of survey research in POM: from constructs to theory},
  author={Malhotra, Manoj K and Grover, Varun},
  journal={Journal of operations management},
  volume={16},
  number={4},
  pages={407--425},
  year={1998},
  publisher={Elsevier}
}

@article{pinsonneault1993survey,
  title={Survey research methodology in management information systems: an assessment},
  author={Pinsonneault, Alain and Kraemer, Kenneth},
  journal={Journal of management information systems},
  volume={10},
  number={2},
  pages={75--105},
  year={1993},
  publisher={Taylor \& Francis}
}

@article{shenton2004strategies,
  title={Strategies for ensuring trustworthiness in qualitative research projects},
  author={Shenton, Andrew K},
  journal={Education for information},
  volume={22},
  number={2},
  pages={63--75},
  year={2004},
  publisher={IOS press}
}

@article{molleri2018cerse,
  title={CERSE-Catalog for empirical research in software engineering: A Systematic mapping study},
  author={Moll{\'e}ri, Jefferson Seide and Petersen, Kai and Mendes, Emilia},
  journal={Information and Software Technology},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{MolleriPM16,
  author    = {Jefferson Seide Moll{\'{e}}ri and
               Kai Petersen and
               Emilia Mendes},
  title     = {Survey Guidelines in Software Engineering: An Annotated Review},
  booktitle = {Proceedings of the 10th {ACM/IEEE} International Symposium on Empirical
               Software Engineering and Measurement, {ESEM} 2016, Ciudad Real, Spain,
               September 8-9, 2016},
  pages     = {58:1--58:6},
  year      = {2016},
}

@article{tong2007consolidated,
  title={Consolidated criteria for reporting qualitative research (COREQ): a 32-item checklist for interviews and focus groups},
  author={Tong, Allison and Sainsbury, Peter and Craig, Jonathan},
  journal={International journal for quality in health care},
  volume={19},
  number={6},
  pages={349--357},
  year={2007},
  publisher={ISQHC}
}

@inproceedings{RodriguezMOT12,
  author    = {Pilar Rodr{\'{\i}}guez and
               Jouni Markkula and
               Markku Oivo and
               Kimmo Turula},
  title     = {Survey on agile and lean usage in finnish software industry},
  booktitle = {2012 {ACM-IEEE} International Symposium on Empirical Software Engineering
               and Measurement, {ESEM} '12, Lund, Sweden - September 19 - 20, 2012},
  pages     = {139--148},
  year      = {2012},
}

@article{pfleeger1995experimental,
	title = {Experimental design and analysis in software engineering},
	volume = {1},
	number = {1},
	journal = {Annals of Software Engineering},
	author = {Pfleeger, Shari Lawrence},
	year = {1995},
	pages = {219--253}
}

@book{babbie1973survey,
	title = {Survey research methods.},
	publisher = {Wadsworth},
	author = {Babbie, Earl R.},
	year = {1973}
}

@book{wohlin2012experimentation,
  author    = {Claes Wohlin and
               Per Runeson and
               Martin H{\"{o}}st and
               Magnus C. Ohlsson and
               Bj{\"{o}}rn Regnell},
  title     = {Experimentation in Software Engineering},
  publisher = {Springer},
  year      = {2012},
}

@book{dawson2005projects,
	title = {Projects in computing and information systems: a student's guide},
	publisher = {Pearson Education},
	author = {Dawson, Christian W.},
	year = {2005}
}

@inproceedings{torchiano2013six,
	title = {Six reasons for rejecting an industrial survey paper},
	booktitle = {Conducting {Empirical} {Studies} in {Industry} ({CESI}), 2013 1st {International} {Workshop} on},
	publisher = {IEEE},
	author = {Torchiano, Marco and Ricca, Filippo},
	year = {2013},
	pages = {21--26}
}

@article{stavru2014critical,
  title={A critical examination of recent industrial surveys on agile method usage},
  author={Stavru, Stavros},
  journal={Journal of Systems and Software},
  volume={94},
  pages={87--97},
  year={2014},
  publisher={Elsevier}
}

@article{yang2016survey,
	title = {A survey on software architectural assumptions},
	volume = {113},
	journal = {Journal of Systems and Software},
	author = {Yang, Chen and Liang, Peng and Avgeriou, Paris},
	year = {2016},
	pages = {362--380}
}

@inproceedings{galster2014exploring,
	title = {Exploring web advertising to attract industry professionals for software engineering surveys},
	booktitle = {Proceedings of the 2nd {International} {Workshop} on {Conducting} {Empirical} {Studies} in {Industry}},
	publisher = {ACM},
	author = {Galster, Matthias and Tofan, Dan},
	year = {2014},
	pages = {5--8}
}

@inproceedings{akbar2012framework,
	title = {A framework of software process tailoring for small and medium size {IT} companies},
	booktitle = {Computer \& {Information} {Science} ({ICCIS}), 2012 {International} {Conference} on},
	publisher = {IEEE},
	author = {Akbar, Rehan and Hassan, Mohd Fadzil and Abdullah, Azrai},
	year = {2012},
	pages = {914--918}
}

@article{bennett2011reporting,
  title={Reporting guidelines for survey research: an analysis of published guidance and reporting practices},
  author={Bennett, Carol and Khangura, Sara and Brehaut, Jamie C and Graham, Ian D and Moher, David and Potter, Beth K and Grimshaw, Jeremy M},
  journal={PLoS Med},
  volume={8},
  number={8},
  pages={e1001069},
  year={2011},
  publisher={Public Library of Science}
}

@book{bourque2003conduct,
  title={How to conduct self-administered and mail surveys},
  author={Bourque, Linda and Fielder, Eve P},
  volume={3},
  year={2003},
  publisher={Sage}
}

@inproceedings{cater2005addressing,
  title={Addressing the challenges of replications of surveys in software engineering research},
  author={Cater-Steel, Aileen and Toleman, Mark and Rout, Terry},
  booktitle={Empirical Software Engineering, 2005. 2005 International Symposium on},
  pages={10--pp},
  year={2005},
  organization={IEEE}
}

@book{ciolkowski2003practical,
  title={Practical experiences in the design and conduct of surveys in empirical software engineering},
  author={Ciolkowski, Marcus and Laitenberger, Oliver and Vegas, Sira and Biffl, Stefan},
  year={2003},
  publisher={Springer}
}

@inproceedings{conradi2005reflections,
  title={Reflections on conducting an international survey of Software Engineering},
  author={Conradi, Reidar and Li, Jingyue and Slyngstad, Odd Petter N and Kampenes, Vigdis By and Bunse, Christian and Morisio, Maurizio and Torchiano, Marco},
  booktitle={Empirical Software Engineering, 2005. 2005 International Symposium on},
  pages={10--pp},
  year={2005},
  organization={IEEE}
}

@inproceedings{de2013would,
  title={Would Sociable Software Engineers Observe Better?},
  author={de Mello, Rafael M and Travassos, Guilherme Horta},
  booktitle={Empirical Software Engineering and Measurement, 2013 ACM/IEEE International Symposium on},
  pages={279--282},
  year={2013},
  organization={IEEE}
}

@inproceedings{de2014sampling,
  title={Sampling improvement in software engineering surveys},
  author={de Mello, Rafael Maiani and da Silva, Pedro Correa and Travassos, Guilherme Horta},
  booktitle={Proceedings of the 8th ACM/IEEE International Symposium on Empirical Software Engineering and Measurement},
  pages={13},
  year={2014},
  organization={ACM}
}

@inproceedings{de2014towards,
  title={Towards a framework to support large scale sampling in software engineering surveys},
  author={de Mello, Rafael Maiani and da Silva, Pedro Correa and Runeson, Per and Travassos, Guilherme Horta},
  booktitle={Proceedings of the 8th ACM/IEEE International Symposium on Empirical Software Engineering and Measurement},
  pages={48},
  year={2014},
  organization={ACM}
}

@inproceedings{de2015characterizing,
  title={Characterizing Sampling Frames in Software Engineering Surveys},
  author={de Mello, Rafael Maiani and Travassos, Guilherme Horta},
  booktitle={Proc. 12th Workshop on Experimental Software Engineering (ESELAW)},
  year={2015}
}

@article{de2015investigating,
  title={Investigating probabilistic sampling approaches for large-scale surveys in software engineering},
  author={de Mello, Rafael Maiani and Da Silva, Pedro Corr{\^e}a and Travassos, Guilherme Horta},
  journal={Journal of Software Engineering Research and Development},
  volume={3},
  number={1},
  pages={1--26},
  year={2015},
  publisher={Springer}
}

@article{dybaa2005empirical,
  title={An empirical investigation of the key factors for success in software process improvement},
  author={Dyb{\aa}, Tore},
  journal={Software Engineering, IEEE Transactions on},
  volume={31},
  number={5},
  pages={410--424},
  year={2005},
  publisher={IEEE}
}

@article{dyba2005evidence,
  title={Evidence-based software engineering for practitioners},
  author={Dyb{\"a}, Tore and Kitchenham, Barbara A and Jorgensen, Magne},
  journal={Software, IEEE},
  volume={22},
  number={1},
  pages={58--65},
  year={2005},
  publisher={IEEE}
}

@book{converse2017survey,
  title={Survey research in the United States: Roots and emergence 1890-1960},
  author={Converse, Jean M},
  year={2017},
  publisher={Routledge}
}

@book{fink2003survey,
  title={The survey handbook},
  author={Fink, Arlene},
  volume={1},
  year={2003},
  publisher={Sage}
}

@book{fowler2013survey,
  title={Survey research methods},
  author={Fowler Jr, Floyd J},
  year={2013},
  publisher={Sage publications}
}

@book{lavrakas2008encyclopedia,
  title={Encyclopedia of survey research methods},
  author={Lavrakas, Paul J},
  year={2008},
  publisher={Sage Publications}
}

@book{alreck1994survey,
  title={The survey research handbook},
  author={Alreck, Pamela L and Settle, Robert B},
  year={1994},
  publisher={McGraw-Hill}
}


@inproceedings{ji2008some,
  title={Some lessons learned in conducting software engineering surveys in china},
  author={Ji, Junzhong and Li, Jingyue and Conradi, Reidar and Liu, Chunnian and Ma, Jianqiang and Chen, Weibing},
  booktitle={Proceedings of the Second ACM-IEEE international symposium on Empirical software engineering and measurement},
  pages={168--177},
  year={2008},
  organization={ACM}
}

@article{kitchenham1997desmet,
  title={DESMET: a methodology for evaluating software engineering methods and tools},
  author={Kitchenham, Barbara and Linkman, Stephen and Law, David},
  journal={Computing \& Control Engineering Journal},
  volume={8},
  number={3},
  pages={120--126},
  year={1997},
  publisher={IET}
}

@article{kitchenham2001principles,
  title={Principles of survey research: parts 1 -- 6},
  author={Kitchenham, Barbara A and Pfleeger, Shari Lawrence},
  journal={ACM SIGSOFT Software Engineering Notes},
  volume={26--28},
  year={2001--2003},
  publisher={ACM}
}

@article{kitchenham2002preliminary,
  title={Preliminary guidelines for empirical research in software engineering},
  author={Kitchenham, Barbara A and Pfleeger, Shari Lawrence and Pickard, Lesley M and Jones, Peter W and Hoaglin, David C and El Emam, Khaled and Rosenberg, Jarrett},
  journal={Software Engineering, IEEE Transactions on},
  volume={28},
  number={8},
  pages={721--734},
  year={2002},
  publisher={IEEE}
}

@incollection{kitchenham2008personal,
  title={Personal opinion surveys},
  author={Kitchenham, Barbara A and Pfleeger, Shari L},
  booktitle={Guide to Advanced Empirical Software Engineering},
  pages={63--92},
  year={2008},
  publisher={Springer}
}

@book{kitchenham2015evidencebased,
  title={Evidence-Based Software Engineering and Systematic Reviews},
  author={Kitchenham, Barbara Ann and Budgen, David and Brereton, Pearl},
  volume={4},
  year={2015},
  pages={234-242},
  publisher={CRC Press}
}

@incollection{kitchenham2015surveys,
  title={Surveys},
  author={Kitchenham, Barbara Ann and Budgen, David and Brereton, Pearl},
  booktitle={Evidence-Based Software Engineering and Systematic Reviews},
  pages={234--242},
  year={2015},
  publisher={CRC Press}
}

@article{linaker2015guidelines,
  title={Guidelines for conducting surveys in software engineering},
  author={Lin{\^A}ker, Johan and Sulaman, Sardar Muhammad and de Mello, R Maiani and Hˆst, Martin and Runeson, P},
  journal={Technical report},
  year={2015}
}

@book{litwin1995measure,
  title={How to measure survey reliability and validity},
  author={Litwin, Mark S},
  volume={7},
  year={1995},
  publisher={Sage Publications}
}

@inproceedings{nugroho2008survey,
  title={A survey into the rigor of UML use and its perceived impact on quality and productivity},
  author={Nugroho, Ariadi and Chaudron, Michel RV},
  booktitle={Proceedings of the Second ACM-IEEE international symposium on Empirical software engineering and measurement},
  pages={90--99},
  year={2008},
  organization={ACM}
}

@inproceedings{petre2013uml,
  title={UML in practice},
  author={Petre, Marian},
  booktitle={Proceedings of the 2013 International Conference on Software Engineering},
  pages={722--731},
  year={2013},
  organization={IEEE Press}
}

@inproceedings{punter2003conducting,
  title={Conducting on-line surveys in software engineering},
  author={Punter, Teade and Ciolkowski, Marcus and Freimut, Bernd and John, Isabel},
  booktitle={Empirical Software Engineering, 2003. ISESE 2003. Proceedings. 2003 International Symposium on},
  pages={80--88},
  year={2003},
  organization={IEEE}
}

@article{rindfleisch2008cross,
  title={Cross-sectional versus longitudinal survey research: Concepts, findings, and guidelines},
  author={Rindfleisch, Aric and Malter, Alan J and Ganesan, Shankar and Moorman, Christine},
  journal={Journal of Marketing Research},
  volume={45},
  number={3},
  pages={261--279},
  year={2008},
  publisher={American Marketing Association}
}

@article{ropponen2000components,
  title={Components of software development risk: how to address them? A project manager survey},
  author={Ropponen, Janne and Lyytinen, Kalle},
  journal={Software Engineering, IEEE Transactions on},
  volume={26},
  number={2},
  pages={98--112},
  year={2000},
  publisher={IEEE}
}

@article{sjoberg2005survey,
  title={A survey of controlled experiments in software engineering},
  author={Sj{\o}berg, Dag IK and Hannay, Jo E and Hansen, Ove and Kampenes, Vigdis By and Karahasanovic, Amela and Liborg, Nils-Kristian and Rekdal, Anette C},
  journal={Software Engineering, IEEE Transactions on},
  volume={31},
  number={9},
  pages={733--753},
  year={2005},
  publisher={IEEE}
}

@article{wieringa2006requirements,
  title={Requirements engineering paper classification and evaluation criteria: a proposal and a discussion},
  author={Wieringa, Roel and Maiden, Neil and Mead, Nancy and Rolland, Colette},
  journal={Requirements Engineering},
  volume={11},
  number={1},
  pages={102--107},
  year={2006},
  publisher={Springer}
}

@article{zhang2013survey,
  title={A survey of experienced user perceptions about software design patterns},
  author={Zhang, Cheng and Budgen, David},
  journal={Information and Software Technology},
  volume={55},
  number={5},
  pages={822--835},
  year={2013},
  publisher={Elsevier}
}

@inproceedings{petersen2013worldviews,
 author = {Petersen, Kai and Gencel, Cigdem},
 title = {Worldviews, Research Methods, and Their Relationship to Validity in Empirical Software Engineering Research},
 booktitle = {Proceedings of the 2013 Joint Conference of the 23Nd International Workshop on Software Measurement (IWSM) and the 8th International Conference on Software Process and Product Measurement},
 series = {IWSM-MENSURA '13},
 year = {2013},
 isbn = {978-0-7695-5078-7},
 pages = {81--89},
 numpages = {9},
 url = {http://dx.doi.org/10.1109/IWSM-Mensura.2013.22},
 doi = {10.1109/IWSM-Mensura.2013.22},
 acmid = {2551833},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
} 

@inproceedings{cruzes2011recommended,
  title={Recommended steps for thematic synthesis in software engineering},
  author={Cruzes, Daniela S and Dyba, Tore},
  booktitle={Empirical Software Engineering and Measurement (ESEM), 2011 International Symposium on},
  pages={275--284},
  year={2011},
  organization={IEEE}
}

@article{contreras2011examining,
  title={Examining the Context in Qualitative Analysis: The Role of the Co-Occurrence Tool in ATLAS. ti},
  author={Contreras, Ricardo B},
  journal={Newsletter},
  volume={2011},
  pages={2},
  year={2011}
}

@article{friese2012atlas,
  title={ATLAS. ti 7 user manual},
  author={Friese, Susanne},
  journal={Berlin: ATLAS. ti Scientific Software Development GmbH},
  year={2012}
}
